Replicating and Scaling up Qualitative Analysis using Crowdsourcing: A Github-based Case Study

Due to the difficulties in replicating and scaling up qualitative studies, such studies are rarely verified. Accordingly, in this paper, we leverage the advantages of crowdsourcing (low costs, fast speed, scalable workforce) to replicate and scale-up one state-of-the-art qualitative study. That qualitative study explored 20 GitHub pull requests to learn factors that influence the fate of pull requests with respect to approval and merging. As a secondary study, using crowdsourcing at a cost of $200, we studied 250 pull requests from 142 GitHub projects. The prior qualitative findings are mapped into questions for crowds workers. Their answers were converted into binary features to build a predictor which predicts whether code would be merged with median F1 scores of 68%. For the same large group of pull requests, the median F1 scores could achieve 90% by a predictor built with additional features defined by prior quantitative results. Based on this case study, we conclude that there is much benefit in combining different kinds of research methods. While qualitative insights are very useful for finding novel insights, they can be hard to scale or replicate. That said, they can guide and define the goals of scalable secondary studies that use (e.g.) crowdsourcing+data mining. On the other hand, while data mining methods are reproducible and scalable to large data sets, their results may be spectacularly wrong since they lack contextual information. That said, they can be used to test the stability and external validity, of the insights gained from a qualitative analysis.

==> Makefile <==
Src=Manuscript#
Bib=$(shell ls *.bib *.bst)#
D=$(HOME)/tmp/$(Src)#
define grab
   gs -sDEVICE=pdfwrite -dNOPAUSE -dBATCH -dSAFER \
       -dFirstPage=$(1) -dLastPage=$(2) \
       -sOutputFile=$@ $<
endef

all: dirs tex bib  tex tex tex     done

typo:
	- git status
	- git commit -am "typo"
	- git push origin master

commit:
	- git status
	- git commit -a
	- git push origin master

update:
	- git pull origin master

status:
	- git status

one: dirs tex done 

open:
	open $(D).pdf

evince:
	evince $(D).pdf 2> /dev/null &


skim:
	/Applications/Skim.app/Contents/MacOS/Skim $(D).pdf &


view:
	evince $(D).pdf &

abe :  $(D)_a.pdf $(D)_b.pdf $(D)_e.pdf

$(D).pdf : $(Src).tex $(Bib)
	pdflatex -output-directory=$(HOME)/tmp $(Src)

$(D)_a.pdf : $(D).pdf; $(call grab,1,1)		
$(D)_b.pdf : $(D).pdf; $(call grab,2,16)		
$(D)_e.pdf : $(D).pdf; $(call grab,18,28)		

done: embedfonts  
	@printf "\n\n\n==============================================\n"
	@printf       "see output in $(D).pdf\n"
	@printf       "==============================================\n\n\n"
	@printf "\n\nWarnings (may be none):\n\n"
	grep arning $D.log

dirs: 
	- [ ! -d $(HOME)/tmp ] && mkdir $(HOME)/tmp

tex: files $(D).pdf

files:
	cp *.tex $(HOME)/tmp

embedfonts:
	@ gs -q -dNOPAUSE -dBATCH -dPDFSETTINGS=/prepress -sDEVICE=pdfwrite \
          -sOutputFile=$(D)-embedded.pdf $(D).pdf
	@ mv  $(D)-embedded.pdf $(D).pdf

bib:
	echo $(Bib)
	- cp $(Bib) $(HOME)/tmp; cd $(HOME)/tmp; bibtex $(Src)
clean:
	rm $D.*


==> method_table.tex <==

  \begin{table}[h!]
  \centering
  \begin{adjustbox}{max width=3.5in}
  \begin{tabular}{|l|l|l|l|}
\hline
\textbf{Methodology} & \textbf{Primary Objective} & \textbf{Primary Data} & \textbf{Design} \\ \hline
Survey               & Descriptive                & Quantitative          & Fixed           \\ \hline
Case Study           & Exploratory                & Qualitative          & Flexible        \\ \hline
Experiments          & Explanatory                & Quantitative          & Fixed           \\ \hline
Action research      & Improving                  & Qualitative           & Flexible        \\ \hline
\end{tabular}
\end{adjustbox}
  \caption{Overview of research methodology characteristics acoording to ~\cite{runeson2009guidelines}}
  \label{tab:method_table}
\end{table}

==> mt_stability.tex <==
\begin{table*}[t!]
\small
	\centering
		\begin{adjustbox}{width=6.6in}
\begin{tabular}{|l|lll|lll|l|}
\cline{1-7}
                                                   & \multicolumn{3}{l|}{\cellcolor[HTML]{C0C0C0}{\color[HTML]{333333} \textbf{Round 1}}}                                                                                                             & \multicolumn{3}{l|}{\cellcolor[HTML]{656565}{\color[HTML]{EFEFEF} \textbf{Round 1 + 2}}}                                                                                                           & \cellcolor[HTML]{343434}{\color[HTML]{FFFFFF} }                                 \\ \cline{2-7}
\multirow{-2}{*}{\textbf{Answers from the Crowd}}  & \cellcolor[HTML]{C0C0C0}{\color[HTML]{333333} \textbf{Yes}} & \cellcolor[HTML]{C0C0C0}{\color[HTML]{333333} \textbf{No}} & \cellcolor[HTML]{C0C0C0}{\color[HTML]{333333} \textbf{\% of Yes (1)}} & \cellcolor[HTML]{656565}{\color[HTML]{EFEFEF} \textbf{Yes}} & \cellcolor[HTML]{656565}{\color[HTML]{EFEFEF} \textbf{No}} & \cellcolor[HTML]{656565}{\color[HTML]{EFEFEF} \textbf{\% of Yes (1+2)}} & \multirow{-2}{*}{\cellcolor[HTML]{343434}{\color[HTML]{FFFFFF} \textbf{$\frac{\text{\% of Yes (1)}}{\text{\% of Yes (1+2)}}$}}} \\ \hline
\textbf{Q1: Show Support?}                          & \textbf{61}                                                 & \textbf{29}                                                & \textbf{67.8\%}                                                       & \textbf{132}                                                & \textbf{58}                                                & \textbf{69.5\%}                                                         & \textbf{0.976}                                                                  \\
Q1: Support from cores.                            & 45                                                          & 44                                                         & 50.6\%                                                                & 111                                                         & 79                                                         & 58.4\%                                                                  & 0.865                                                                           \\
Q1: Support from externals.                        & 26                                                          & 64                                                         & 28.9\%                                                                & 35                                                          & 155                                                        & 18.4\%                                                                  & 1.568                                                                           \\ \hline
\textbf{Q2: Propose Alternate Solution?}                   & \textbf{58}                                                 & \textbf{32}                                                & \textbf{64.4\%}                                                       & \textbf{119}                                                & \textbf{71}                                                & \textbf{62.6\%}                                                         & \textbf{1.029}                                                                  \\
Q2: Alternate solution from cores.                 & 46                                                          & 44                                                         & 51.1\%                                                                & 92                                                          & 98                                                         & 48.4\%                                                                  & 1.056                                                                           \\
Q2: Alternate solution from externals.             & 18                                                          & 72                                                         & 20.0\%                                                                & 36                                                          & 153                                                        & 19.0\%                                                                  & 1.050                                                                           \\ \hline
\textbf{Q3: Disapprove the Solution?}               & \textbf{42}                                                 & \textbf{48}                                                & \textbf{46.7\%}                                                       & \textbf{86}                                                 & \textbf{103}                                               & \textbf{45.5\%}                                                         & \textbf{1.026}                                                                  \\
Q3: Bugs.                                          & 12                                                          & 78                                                         & 13.3\%                                                                & 31                                                          & 158                                                        & 16.4\%                                                                  & 0.813                                                                           \\
Q3: Consistency.                                   & 11                                                          & 78                                                         & 12.4\%                                                                & 22                                                          & 167                                                        & 11.6\%                                                                  & 1.062                                                                           \\
Q3: Need improvement.                              & 27                                                          & 62                                                         & 30.3\%                                                                & 50                                                          & 139                                                        & 26.5\%                                                                  & 1.147                                                                           \\ \hline
\textbf{Q4: Disapprove the Problems Being Solved?} & \textbf{18}                                                 & \textbf{72}                                                & \textbf{20.0\%}                                                       & \textbf{45}                                                 & \textbf{144}                                               & \textbf{23.8\%}                                                         & \textbf{0.840}                                                                  \\
Q4: Doesn't fit the project.                       & 4                                                           & 85                                                         & 4.5\%                                                                 & 11                                                          & 178                                                        & 5.8\%                                                                   & 0.772                                                                           \\
Q4: Solution has no value.                         & 10                                                          & 80                                                         & 11.1\%                                                                & 29                                                          & 160                                                        & 15.3\%                                                                  & 0.724                                                                           \\ \hline
\textbf{Total}                                     & \textbf{378}                                                & \textbf{788}                                               & \textbf{32.4\%}                                                       & \textbf{799}                                                & \textbf{1663}                                              & \textbf{32.5\%}                                                         & \textbf{0.999}                                                                  \\ \hline
\end{tabular}
		\end{adjustbox}
	\caption{Stability for Crowdsourcing Results from Amazon Mechanical Turk.}
	\label{mt_stability}
    \end{table*}
    
